Giant Rashba electrical control of magnetism in band models

It is of considerable technological importance to achieve an electrical control of magnetism of sufficient magnitude. To overcome the in-plane shape anisotropy, needed is the electrical control of a perpendicular magnetic anisotropy (PMA). It is known, within a free electron model, the Rashba spin-orbit coupling provides such a control. Surprisingly, this same Rashba PMA is enhanced by two to three orders of magnitude when a periodic potential is added. Usually spin Berry phase physics reflects time dependent magnetic fields. Here it is shown, within a time independent model, such physics arises because the Rashba effective magnetic field has texture within the unit cell. Predicted are electrical controllable band-structure gaps, linear in the applied electric field $E$, that can result in a truly giant linear PMA. Also possible is a Peierls mechanism, in which the magnetisation tilts from the vertical, shifting these gaps to the Fermi level. As a consequence there are low dissipation electric field driven dynamics, an alternative to the more dissipative spin torque transfer (STT) effect. The theory requires the introduction of an intrinsic spin Berry connection $\vec A_s$, an effective vector potential, and is incompatible with current density functional theories (DFT).

==> citationBibitem.tex <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{\url{https://doi.org/#1}}
\bibcommenthead

\bibitem{Wang2020}
L.~Wang, X.~Li, T.~Sasaki, K.~Wong, G.~Yu, S.~Peng, C.~Zhao, T.~Ohkubo,
  K.~Hono, W.~Zhao, K.~Wang, High voltage-controlled magnetic anisotropy and
  interface magnetoelectric effect in sputtered multilayers annealed at high
  temperatures.
\newblock Science China Physics, Mechanics {\&} Astronomy \textbf{63}(7),
  277,512 (2020).
\newblock \doi{10.1007/s11433-019-1524-y}.
\newblock \urlprefix\url{https://doi.org/10.1007/s11433-019-1524-y}

\bibitem{Barnes2014}
S.E. Barnes, J.~Ieda, S.~Maekawa, Rashba spin-orbit anisotropy and the electric
  field control of magnetism.
\newblock Scientific Reports \textbf{4}(1), 4105 (2014).
\newblock \doi{10.1038/srep04105}.
\newblock \urlprefix\url{https://doi.org/10.1038/srep04105}

\bibitem{Barnes2012}
S.E. Barnes, in \emph{Spin Current}, ed. by S.~Maekawa, S.O. Valenzuela,
  E.~Saitoh, T.~Kimura (Oxford Scholarship, 2013), chap.~7

\bibitem{Gruner1988}
G.~Gr\"uner, The dynamics of charge-density waves.
\newblock Rev. Mod. Phys. \textbf{60}, 1129--1181 (1988).
\newblock \doi{10.1103/RevModPhys.60.1129}.
\newblock \urlprefix\url{https://link.aps.org/doi/10.1103/RevModPhys.60.1129}

\bibitem{Barnes1983}
S.E. Barnes, A.~Zawadowski, Theory of josephson-type oscillations in a moving
  charge-density wave.
\newblock Phys. Rev. Lett. \textbf{51}, 1003--1006 (1983).
\newblock \doi{10.1103/PhysRevLett.51.1003}.
\newblock \urlprefix\url{https://link.aps.org/doi/10.1103/PhysRevLett.51.1003}

\bibitem{Slonczewski1996}
J.~Slonczewski, Current-driven excitation of magnetic multilayers.
\newblock Journal of Magnetism and Magnetic Materials \textbf{159}(1), L1--L7
  (1996).
\newblock \doi{https://doi.org/10.1016/0304-8853(96)00062-5}.
\newblock
  \urlprefix\url{https://www.sciencedirect.com/science/article/pii/0304885396000625}

\bibitem{Messiah1966}
A.~Messiah, \emph{Quantum Mechanics} (Dover Publications, 2014)

\bibitem{FW1950}
L.L. Foldy, S.A. Wouthuysen, On the dirac theory of spin 1/2 particles and its
  non-relativistic limit.
\newblock Phys. Rev. \textbf{78}, 29--36 (1950).
\newblock \doi{10.1103/PhysRev.78.29}.
\newblock \urlprefix\url{https://link.aps.org/doi/10.1103/PhysRev.78.29}

\bibitem{Winkler2003}
R.~Winkler, \emph{Spin-orbit coupling effects in two-dimensional electron and
  Hole Systems} (Springer, 2011)

\bibitem{Wang1996}
X.~Wang, R.~Wu, D.s. Wang, A.J. Freeman, Torque method for the theoretical
  determination of magnetocrystalline anisotropy.
\newblock Phys. Rev. B \textbf{54}, 61--64 (1996).
\newblock \doi{10.1103/PhysRevB.54.61}.
\newblock \urlprefix\url{https://link.aps.org/doi/10.1103/PhysRevB.54.61}

\bibitem{Rashba1984}
Y.A. {Bychkov}, {\'E}.I. {Rashba}, {Properties of a 2D electron gas with lifted
  spectral degeneracy}.
\newblock Soviet Journal of Experimental and Theoretical Physics Letters
  \textbf{39}, 78 (1984)

\bibitem{Ong2015}
P.V. Ong, N.~Kioussis, D.~Odkhuu, P.~Khalili~Amiri, K.L. Wang, G.P. Carman,
  Giant voltage modulation of magnetic anisotropy in strained heavy
  metal/magnet/insulator heterostructures.
\newblock Phys. Rev. B \textbf{92}, 020,407 (2015).
\newblock \doi{10.1103/PhysRevB.92.020407}.
\newblock \urlprefix\url{https://link.aps.org/doi/10.1103/PhysRevB.92.020407}

\bibitem{Yao2004}
Y.~Yao, L.~Kleinman, A.H. MacDonald, J.~Sinova, T.~Jungwirth, D.s. Wang,
  E.~Wang, Q.~Niu, First principles calculation of anomalous hall conductivity
  in ferromagnetic bcc fe.
\newblock Phys. Rev. Lett. \textbf{92}, 037,204 (2004).
\newblock \doi{10.1103/PhysRevLett.92.037204}.
\newblock
  \urlprefix\url{https://link.aps.org/doi/10.1103/PhysRevLett.92.037204}

\bibitem{Manchon2015}
A.~Manchon, H.C. Koo, J.~Nitta, S.M. Frolov, R.A. Duine, New perspectives for
  rashba spin--orbit coupling.
\newblock Nature Materials \textbf{14}(9), 871--882 (2015).
\newblock \doi{10.1038/nmat4360}.
\newblock \urlprefix\url{https://doi.org/10.1038/nmat4360}

\bibitem{Blaha2001}
P.~Blaha, K.~Schwarz, G.~Madsen, D.~Kvasnicka, J.~Luitz, R.~Laskowsk, F.~Tran,
  L.~Marks, L.~Marks, \emph{WIEN2k: An Augmented Plane Wave Plus Local Orbitals
  Program for Calculating Crystal Properties} (Techn. Universitat, 2019)

\bibitem{Kresse1993a}
D.~Hobbs, G.~Kresse, J.~Hafner, Fully unconstrained noncollinear magnetism
  within the projector augmented-wave method.
\newblock Phys. Rev. B \textbf{62}, 11,556--11,570 (2000).
\newblock \doi{10.1103/PhysRevB.62.11556}.
\newblock \urlprefix\url{https://link.aps.org/doi/10.1103/PhysRevB.62.11556}

\bibitem{Kresse1993b}
G.~Kresse, J.~Furthm\"uller, Efficient iterative schemes for ab initio
  total-energy calculations using a plane-wave basis set.
\newblock Phys. Rev. B \textbf{54}, 11,169--11,186 (1996).
\newblock \doi{10.1103/PhysRevB.54.11169}.
\newblock \urlprefix\url{https://link.aps.org/doi/10.1103/PhysRevB.54.11169}

\bibitem{Kresse1993c}
G.~Kresse, J.~Furthmüller, Efficiency of ab-initio total energy calculations
  for metals and semiconductors using a plane-wave basis set.
\newblock Computational Materials Science \textbf{6}(1), 15--50 (1996).
\newblock \doi{https://doi.org/10.1016/0927-0256(96)00008-0}.
\newblock
  \urlprefix\url{https://www.sciencedirect.com/science/article/pii/0927025696000080}

\bibitem{Kresse1993d}
D.~Hobbs, G.~Kresse, J.~Hafner, Fully unconstrained noncollinear magnetism
  within the projector augmented-wave method.
\newblock Phys. Rev. B \textbf{62}, 11,556--11,570 (2000).
\newblock \doi{10.1103/PhysRevB.62.11556}.
\newblock \urlprefix\url{https://link.aps.org/doi/10.1103/PhysRevB.62.11556}

\bibitem{Koseki2019}
S.~Koseki, N.~Matsunaga, T.~Asada, M.W. Schmidt, M.S. Gordon, Spin–orbit
  coupling constants in atoms and ions of transition elements: Comparison of
  effective core potentials, model core potentials, and all-electron methods.
\newblock The Journal of Physical Chemistry A \textbf{123}(12), 2325--2339
  (2019).
\newblock \doi{10.1021/acs.jpca.8b09218}.
\newblock \urlprefix\url{https://doi.org/10.1021/acs.jpca.8b09218}.
\newblock PMID: 30817150.
\newblock
  {\href{https://arxiv.org/abs/https://doi.org/10.1021/acs.jpca.8b09218}{{https://doi.org/10.1021/acs.jpca.8b09218}}}

\bibitem{Landau1991}
L.L. Davidovič, L.E. M., \emph{@Quantum mechanics non-relativistic theory}
  (Butterworth Heinemann, 1991)

\bibitem{SupMat}
See the supplementary materials for details of the calculations.

\bibitem{radialint}
The integral $\langle \frac{1}{r^3} \rangle = \frac{Z^3}{n^3\ell(\ell +
  \frac{1}{2})(\ell+1)} \frac{1}{{a_0}^3} $, so if $\ell = 1$ then $n=2$ and
  there is an additional factor of $\frac{1}{n^3\ell(\ell +
  \frac{1}{2})(\ell+1)} = \frac{1}{24}$. for the estimation of the electric
  field $\langle \frac{1}{r^2} \rangle =\frac{2Z^2}{n^3(2\ell+1) {a_0}^2} $ is
  used

\bibitem{Shankar1994}
R.~Shankar, \emph{Principles of Quantum Mechanics} (Springer, 2014)

\bibitem{Berry1984}
M.V. {Berry}, {Quantal Phase Factors Accompanying Adiabatic Changes}.
\newblock Proceedings of the Royal Society of London Series A
  \textbf{392}(1802), 45--57 (1984).
\newblock \doi{10.1098/rspa.1984.0023}

\bibitem{Ye2001a}
J.~Ye, Y.B. Kim, A.J. Millis, B.I. Shraiman, P.~Majumdar, Z.~Te\ifmmode
  \check{s}\else \v{s}\fi{}anovi\ifmmode~\acute{c}\else \'{c}\fi{}, Berry phase
  theory of the anomalous hall effect: Application to colossal
  magnetoresistance manganites.
\newblock Phys. Rev. Lett. \textbf{83}, 3737--3740 (1999).
\newblock \doi{10.1103/PhysRevLett.83.3737}.
\newblock \urlprefix\url{https://link.aps.org/doi/10.1103/PhysRevLett.83.3737}

\bibitem{Ye2001b}
Y.~Taguchi, Y.~Oohara, H.~Yoshizawa, N.~Nagaosa, Y.~Tokura, Spin chirality,
  berry phase, and anomalous hall effect in a frustrated ferromagnet.
\newblock Science \textbf{291}, 2573–2576 (2001).
\newblock \doi{10.1126/science.1058161}

\bibitem{Ye2001c}
R.~Shindou, N.~Nagaosa, Orbital ferromagnetism and anomalous hall effect in
  antiferromagnets on the distorted fcc lattice.
\newblock Phys. Rev. Lett. \textbf{87}, 116,801 (2001).
\newblock \doi{10.1103/PhysRevLett.87.116801}.
\newblock
  \urlprefix\url{https://link.aps.org/doi/10.1103/PhysRevLett.87.116801}

\bibitem{Kronig1931}
R.D.L. Kronig, W.G. Penney, R.H. Fowler, Quantum mechanics of electrons in
  crystal lattices.
\newblock Proceedings of the Royal Society of London. Series A, Containing
  Papers of a Mathematical and Physical Character \textbf{130}(814), 499--513
  (1931).
\newblock \doi{10.1098/rspa.1931.0019}.
\newblock
  \urlprefix\url{https://royalsocietypublishing.org/doi/abs/10.1098/rspa.1931.0019}.
\newblock
  {\href{https://arxiv.org/abs/https://royalsocietypublishing.org/doi/pdf/10.1098/rspa.1931.0019}{{https://royalsocietypublishing.org/doi/pdf/10.1098/rspa.1931.0019}}}

\bibitem{Nearing}
J.~Nearing.
\newblock Unpublished

\bibitem{Tight}
V.~Rosato, M.~Guillope, B.~Legrand.
\newblock Thermodynamical and structural properties of f.c.c. transition metals
  using a simple tight-binding model (1989).
\newblock \doi{10.1080/01418618908205062}.
\newblock
  \urlprefix\url{https://www.tandfonline.com/doi/abs/10.1080/01418618908205062}

\bibitem{Stoner1948}
E.C. Stoner, E.P. Wohlfarth, A mechanism of magnetic hysteresis in
  heterogeneous alloys.
\newblock Philosophical Transactions of the Royal Society of London. Series A,
  Mathematical and Physical Sciences \textbf{240}(826), 599--642 (1948).
\newblock \doi{10.1098/rsta.1948.0007}.
\newblock
  \urlprefix\url{https://royalsocietypublishing.org/doi/abs/10.1098/rsta.1948.0007}.
\newblock
  {\href{https://arxiv.org/abs/https://royalsocietypublishing.org/doi/pdf/10.1098/rsta.1948.0007}{{https://royalsocietypublishing.org/doi/pdf/10.1098/rsta.1948.0007}}}

\bibitem{Lau2019}
Y.C. Lau, Z.~Chi, T.~Taniguchi, M.~Kawaguchi, G.~Shibata, N.~Kawamura,
  M.~Suzuki, S.~Fukami, A.~Fujimori, H.~Ohno, M.~Hayashi, Giant perpendicular
  magnetic anisotropy in ir/co/pt multilayers.
\newblock Phys. Rev. Materials \textbf{3}, 104,419 (2019).
\newblock \doi{10.1103/PhysRevMaterials.3.104419}.
\newblock
  \urlprefix\url{https://link.aps.org/doi/10.1103/PhysRevMaterials.3.104419}

\bibitem{Luttinger1954}
R.~Karplus, J.M. Luttinger, Hall effect in ferromagnetics.
\newblock Phys. Rev. \textbf{95}, 1154--1160 (1954).
\newblock \doi{10.1103/PhysRev.95.1154}.
\newblock \urlprefix\url{https://link.aps.org/doi/10.1103/PhysRev.95.1154}

\bibitem{MacDonald2018}
G.~Chaudhary, M.d.S. Dias, A.H. MacDonald, S.~Lounis, Anatomy of magnetic
  anisotropy induced by rashba spin-orbit interactions.
\newblock Phys. Rev. B \textbf{98}, 134,404 (2018).
\newblock \doi{10.1103/PhysRevB.98.134404}.
\newblock \urlprefix\url{https://link.aps.org/doi/10.1103/PhysRevB.98.134404}

\bibitem{Lieb1983}
E.H. Lieb, Density functionals for coulomb systems.
\newblock International Journal of Quantum Chemistry \textbf{24}(3), 243--277
  (1983).
\newblock \doi{https://doi.org/10.1002/qua.560240302}.
\newblock
  \urlprefix\url{https://onlinelibrary.wiley.com/doi/abs/10.1002/qua.560240302}.
\newblock
  {\href{https://arxiv.org/abs/https://onlinelibrary.wiley.com/doi/pdf/10.1002/qua.560240302}{{https://onlinelibrary.wiley.com/doi/pdf/10.1002/qua.560240302}}}

\bibitem{Hohenberg1964}
P.~Hohenberg, W.~Kohn, Inhomogeneous electron gas.
\newblock Phys. Rev. \textbf{136}, B864--B871 (1964).
\newblock \doi{10.1103/PhysRev.136.B864}.
\newblock \urlprefix\url{https://link.aps.org/doi/10.1103/PhysRev.136.B864}

\bibitem{Kohn1965}
W.~Kohn, L.J. Sham, Self-consistent equations including exchange and
  correlation effects.
\newblock Phys. Rev. \textbf{140}, A1133--A1138 (1965).
\newblock \doi{10.1103/PhysRev.140.A1133}.
\newblock \urlprefix\url{https://link.aps.org/doi/10.1103/PhysRev.140.A1133}

\bibitem{Kohn2004}
W.~Kohn, A.~Savin, C.A. Ullrich, Hohenberg–kohn theory including spin
  magnetism and magnetic fields.
\newblock International Journal of Quantum Chemistry \textbf{101}(5), 20--21
  (2005).
\newblock \doi{https://doi.org/10.1002/qua.20303}.
\newblock
  \urlprefix\url{https://onlinelibrary.wiley.com/doi/abs/10.1002/qua.20303}.
\newblock
  {\href{https://arxiv.org/abs/https://onlinelibrary.wiley.com/doi/pdf/10.1002/qua.20303}{{https://onlinelibrary.wiley.com/doi/pdf/10.1002/qua.20303}}}

\bibitem{Vignale1988}
G.~Vignale, M.~Rasolt, Current- and spin-density-functional theory for
  inhomogeneous electronic systems in strong magnetic fields.
\newblock Phys. Rev. B \textbf{37}, 10,685--10,696 (1988).
\newblock \doi{10.1103/PhysRevB.37.10685}.
\newblock \urlprefix\url{https://link.aps.org/doi/10.1103/PhysRevB.37.10685}

\bibitem{Janecek2013}
S.~Janecek, M.~Aichinger, E.R. Hern\'andez, Two-dimensional bloch electrons in
  perpendicular magnetic fields: An exact calculation of the hofstadter
  butterfly spectrum.
\newblock Phys. Rev. B \textbf{87}, 235,429 (2013).
\newblock \doi{10.1103/PhysRevB.87.235429}.
\newblock \urlprefix\url{https://link.aps.org/doi/10.1103/PhysRevB.87.235429}

\bibitem{Adler2019}
R.~Adler, C.J. Kang, C.H. Yee, G.~Kotliar, Correlated materials design:
  prospects and challenges.
\newblock Reports on Progress in Physics \textbf{82}(1), 012,504 (2018).
\newblock \doi{10.1088/1361-6633/aadca4}.
\newblock \urlprefix\url{https://doi.org/10.1088%2F1361-6633%2Faadca4}

\end{thebibliography}

